Communication Trade-offs in Federated Learning of Spiking Neural Networks

Spiking Neural Networks (SNNs) are biologically inspired alternatives to conventional Artificial Neural Networks (ANNs). Despite promising preliminary results, the trade-offs in the training of SNNs in a distributed scheme are not well understood. Here, we consider SNNs in a federated learning setting where a high-quality global model is created by aggregating multiple local models from the clients without sharing any data. We investigate federated learning for training multiple SNNs at clients when two mechanisms reduce the uplink communication cost: i) random masking of the model updates sent from the clients to the server; and ii) client dropouts where some clients do not send their updates to the server. We evaluated the performance of the SNNs using a subset of the Spiking Heidelberg digits (SHD) dataset. The results show that a trade-off between the random masking and the client drop probabilities is crucial to obtain a satisfactory performance for a fixed number of clients.

==> extras.tex <==
% There are scopes of research to investigate the performance of SNNs in FL setup, especially with unreliable connections. The costs for uplink and downlink communications between the server and the nodes can be expensive in a FL setup. So, it would be interesting to explore the possibilities to reduce this cost without compromising the performance of the federated SNNs to a great extent.



% \\ \textcolor{red}{Aim of this work + novelty}


 We explore the performances of the high-quality global models with varying number of clients over computation rounds. Also, unreliable connection between the server and the nodes along with the communication costs between them are bottlenecks of federated implementations. Therefore, we have investigate these scenarios with introducing a dropping probability of the clients and restricting the updates to be a sparse matrix during uplink communication. 
 \\ \textcolor{red}{Novelty List
 \begin{itemize}
     \item Reduced uplink communication cost by sending randomly masked weight updates from the clients to the server
     \item Investigated performances of the federated SNNs with unreliable connections
     \item Performances of federated SNNs using SHD-5 class dataset (not really a novelty, most SL+FNN papers reported results with CIFAR10, CIFAR100 \cite{Venkatesha2021}, MNIST-DVS dataset \cite{Skatchkovsky2020}, and the BelgiumTS dataset \cite{xie2022})
 \end{itemize}}


 % \\ In this paper, we design a framework for federated SNNs and implement it on a benchmarked dataset \textemdash Spiking Heidelberg digits (SHD).
